"Look Ma, No Hands!" A Parameter-Free Topic Model

It has always been a burden to the users of statistical topic models to predetermine the right number of topics, which is a key parameter of most topic models. Conventionally, automatic selection of this parameter is done through either statistical model selection (e.g., cross-validation, AIC, or BIC) or Bayesian nonparametric models (e.g., hierarchical Dirichlet process). These methods either rely on repeated runs of the inference algorithm to search through a large range of parameter values which does not suit the mining of big data, or replace this parameter with alternative parameters that are less intuitive and still hard to be determined. In this paper, we explore to "eliminate" this parameter from a new perspective. We first present a nonparametric treatment of the PLSA model named nonparametric probabilistic latent semantic analysis (nPLSA). The inference procedure of nPLSA allows for the exploration and comparison of different numbers of topics within a single execution, yet remains as simple as that of PLSA. This is achieved by substituting the parameter of the number of topics with an alternative parameter that is the minimal goodness of fit of a document. We show that the new parameter can be further eliminated by two parameter-free treatments: either by monitoring the diversity among the discovered topics or by a weak supervision from users in the form of an exemplar topic. The parameter-free topic model finds the appropriate number of topics when the diversity among the discovered topics is maximized, or when the granularity of the discovered topics matches the exemplar topic. Experiments on both synthetic and real data prove that the parameter-free topic model extracts topics with a comparable quality comparing to classical topic models with "manual transmission". The quality of the topics outperforms those extracted through classical Bayesian nonparametric models.

==> abstract.tex <==
%contribution:(1) the NPLSA algorithm (2) Diversity  (3) User-query induced 
%Story: Minimizing User Effort in Topic Modeling
%(1) effective and efficient
%(2) automatically infer the number of topics
%(3) provides user-customized way.
\begin{abstract}
A fundamental problem in the field of topic modeling is to determine the number of topics within the corpus. Along this direction, Bayesian nonparametric models such as Dirichlet process mixture, which can model infinite mixtures and hence adapt the number of topics to the complexity of the data, have become quite popular. However, these models tend to have sophisticated inference procedure and hard to scale up, both of which substantially prevents their usability in practice.

In this paper, we proposed a nonparametric topic model  Nonparametric Probabilistic Latent Semantic Analysis (NPLSA), which is built on top of the classical simple and efficient model probabilistic latent semantic analysis (PLSA). The NPLSA model shares similar Expectation-Maximization (EM) iterative procedure for PLSA except that it allows to generate new topics in E-step. We prove that the underlying objective function of the algorithm is actually the log-likelihood of the data penalized by the number of topics. We further proposed two criteria for stopping generating new topics based on the diversity of existing topics or some weak supervision from users in the form of some keywords. Through experiments on synthetic dataset, the model can find the exact number of topics and achieve comparable performance with state-of-the-art topic models PLSA and Latent Dirichlet Allocation (LDA). Experiments on real world dataset also shows promising performance in terms of model fitting, topic quality and diversity. 
\end{abstract}

%%%version 2
\begin{abstract}
Topic modeling is important for discovering semantic structure within the data for further data exploration. A good topic modeling tool should satisfy the following three conditions: (1) it should be effective and efficient; (2) it can automatically adapt the number of topics to the data; (3) it allows users to provide some weak supervision to customize the topics.

In this paper, we proposed a  topic model named Nonparametric Probabilistic Latent Semantic Analysis (NPLSA) which can satisfy all the above three conditions. First, the NPLSA model shares similar learning procedure with the classical PLSA model,  and it is both effective and efficient. But it allows to generate a new topic during the learning process when existing topics cannot accommodate a new document. This process turns out to be monotonically maximizing the log-likelihood of the training data penalized by the number of topics.   Second, through our experiments on synthetic data, we found that the diversity between the topics optimized upon discovering the right number of topics. Based on it, we can make the algorithm stop generating new topics. Third,  we provided a way to allow users to customize the size of the desired topics in the form of some keywords. Experiments on both synthetic and real data showed promising performance in terms of discovering the right number of topics, topic quality, diversity and user customizability.
\end{abstract}

Title: Listen to the Data and User: Adaptive Topic Modeling

Title: Look Mum No Hands: A Parameter-Free Topic Model

==> metrics.tex <==

\section{Evaluation Metrics}
In this section, we define some metrics for evaluating the quality of the topics. In the experiment part, we evaluated the models on both the synthetic and real world datasets. For the synthetic dataset, we known the ground truth of the topics. Let the ground truth topics be $\Theta=\{\theta_k\}_{k=1,\ldots K}$, and the learned topics be $\tilde{\Theta}=\{\tilde{\theta}_j\}_{j=1,\ldots \tilde{K}}$, where $K, \tilde{K}$ are the number of ground truth topics and the learned topics respectively. First, we define two metrics in the case of knowing the ground truth topics.

\begin{mydef}
\textbf{Topic Quality Error} measures the quality of the learned topics against the ground truth topics. The quality error of each individual learned topic is defined as the minimum distance between the topic and the ground truth topics. The overall topic quality error is averaged over the learned topics and formulated as:
\begin{equation}
  \text{TQE}=\frac{1}{\tilde{K}}\sum_{j=1}^{\tilde{K}}\min_{k=1,\ldots K}l_2(\tilde{\theta}_j, \theta_k)
\end{equation}
\end{mydef}
where $l_2(\cdot,\cdot)$ is the Euclidean distance between two real-value vectors.

Topic quality error only measures the quality of learned topics. However, even the topic quality of each individual learned topic is quite good, if they are duplicated with each other, the underlying topics may still not be well covered by the learned topics. Hence, we further introduce to measure the coverage of the learned topics. 
\begin{mydef}
\textbf{Topic Coverage Error} measures the error of the learned topics in covering the ground truth topics. The error of each individual ground truth topic covered by the learned topics is defined as the minimum distance between the topic and the learned topics. The overall coverage error is averaged over the ground truth topics and formulated as:
\begin{equation}
  \text{TCE}=\frac{1}{K}\sum_{k=1}^{K}\min_{j=1,\ldots \tilde{K}}l_2(\theta_k,\tilde{\theta}_j)
\end{equation}
\end{mydef}

The above two metrics both rely on the ground truth of the topics. However, for real world datasets, we do not know the ground truth. In the following, we introduce two metrics that do not depend on the ground truth of the topics. 

In real practice, the discovered topics are often used for data exploration. Thus the topics should be interpretable, i.e the topics should be semantic coherence. Evaluating the semantic coherence of the topics is receiving increasing attention for topic modeling evaluation~\cite{DBLP:conf/jcdl/NewmanNTKB10,newman2010automatic,DBLP:conf/emnlp/MimnoWTLM11}. In~\cite{DBLP:conf/jcdl/NewmanNTKB10,newman2010automatic}, Newman et al. proposed to use Point-wise Mutual Information (PMI) to measure the semantic coherence of topics. 
\begin{mydef}
\textbf{Topic Semantic Coherence} is used to measure the semantic coherence of the learned topics. For each topic, the semantic coherence is defined as the average point-wise mutual information score of the word pairs in top-N ranked words $\mathbf{w}$ in the topic:
\begin{equation}
\begin{aligned}
  \text{PMI}(\mathbf{w})=\frac{2}{N(N-1)}\sum_{i<j}\log \frac{p(w_i,w_j)}{p(w_i)p(w_j)},\\
  i,j\in\{1,\ldots,N\}
\end{aligned}
\end{equation}
\end{mydef}
where $\mathbf{w}$ are the top $N$ most probable words of the topic. $p(w_i, w_j)$ is the probability of the word pair $w_i$ and $w_j$ co-occuring in the same document while $p(w_i)$ is probability of word $w_i$ appearing in a single document. In our experiments, $N$ is set to 20. To calculate the PMI score,  an external large dataset is required to calculate the point-wise mutual information between the words. 



==> plsa.tex <==
\section{PLSA}
A classical parametric topic model, probabilistic latent semantic analysis (PLSA), assumes that each document is a mixture proportion of topics, with each topic corresponding to a multinomial distribution over the word vocabulary. The log-likelihood $L(D)$ of the training data $D$ is calculated by:
\begin{equation}
\label{plsa:likelihood}
  L(D)=\sum_d\sum_w n(d,w)\log\sum_z p(z|d)p(w|z).
\end{equation}
where $n(d,w)$ is the word frequency $w$ in document $d$, $p(z|d)$ is the probability of topic $z$ in document $d$, and $p(w|z)$ is the probability of word $w$ generated by topic $z$.
Following the maximum-likelihood principle, the parameters of the model, i.e. $p(z|d)$, and $p(w|z)$,  are estimated by maximizing the log-likelihood objective function (1). Due to the non-convexity of the log-likelihood defined by (1), it is difficult to obtain the global optimum value. To this end, EM algorithm is generally applied for the problem. The EM algorithm alternates between two steps: E-step and M-step. In the E-step, it calculates the posterior distribution of the latent variable z conditioned on the observation and current model parameters. In the M-step, it updates the model parameters based on the posterior probability calculated in the E-step. We summarize the detailed updating equations as below:

\textbf{E-step:} computing the posterior of the latent variable $p(z|d,w)$ as follows:
\begin{equation}
  p(z|d,w)=\frac{p(z|d)p(w|z)}{\sum_z' p(z'|d)p(w|z')}
\end{equation}
	
    \textbf{M-step:} updating the model parameters $p(z|d)$ and $p(w|z)$ based on the E-step:
\begin{equation}
  p(z|d)\propto \sum_w n(d,w)p(z|d,w)
\end{equation}
\begin{equation}
  p(w|z) \propto \sum_d n(d,w)p(z|d,w)
\end{equation}

In order to apply PLSA for topic modeling, users are required to specify the number of topics, $K$. However, it is generally quite hard for a user to estimate the number of topics in his dataset a priori, which brings a considerable burden to the user. In this paper, we aim to get rid of the parameter $K$ and help reduce users' effort when practicing topic models. In the next section, we introduce our methods to eliminate the parameter $K$. 
